FactCHD: Benchmarking Fact-Conflicting Hallucination Detection

Despite their impressive generative capabilities, LLMs are hindered by fact-conflicting hallucinations in real-world applications. The accurate identification of hallucinations in texts generated by LLMs, especially in complex inferential scenarios, is a relatively unexplored area. To address this gap, we present FactCHD, a dedicated benchmark designed for the detection of fact-conflicting hallucinations from LLMs. FactCHD features a diverse dataset that spans various factuality patterns, including vanilla, multi-hop, comparison, and set operation. A distinctive element of FactCHD is its integration of fact-based evidence chains, significantly enhancing the depth of evaluating the detectors' explanations. Experiments on different LLMs expose the shortcomings of current approaches in detecting factual errors accurately. Furthermore, we introduce Truth-Triangulator that synthesizes reflective considerations by tool-enhanced ChatGPT and LoRA-tuning based on Llama2, aiming to yield more credible detection through the amalgamation of predictive results and evidence. The benchmark dataset is available at https://github.com/zjunlp/FactCHD.

==> Section/0_define.tex <==

\definecolor{green}{rgb}{0.1,0.1,0.1}
\definecolor{chocolate}{HTML}{D2691E}
\definecolor{maroon}{HTML}{A00000}
\definecolor{indigo}{HTML}{4B0082}
\definecolor{green}{HTML}{008000}
\definecolor{red}{HTML}{a91e1e}
\definecolor{cadmiumgreen}{rgb}{0.0, 0.42, 0.24}
\newcommand{\mydarkgreen}[1]{\textcolor{cadmiumgreen}{#1}}
\newcommand{\best}[1]{\textcolor{red}{\textbf{#1}}}

\DeclareMathOperator*{\argmax}{argmax} 
\DeclareMathOperator*{\argtopk}{argTopk} 
\newcolumntype{L}[1]{>{\PreserveBackslash\raggedright}p{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\usepackage{amssymb}% http://ctan.org/pkg/amssymb
\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{{\protect\color{maroon} \ding{51}}}
\newcommand{\xmark}{\ding{55}}
\newcommand{\gmark}{{\protect\color{ForestGreen} \ding{51}}}
\makeatletter
\newcommand*\myfontsize{%
  \@setfontsize\myfontsize{8}{9}%
}
\makeatother


\makeatletter
\newcommand*\mysmallfontsize{%
  \@setfontsize\mysmallfontsize{7.4}{8.4}%
}
\makeatother





%\newcommand{\ours}{\textsc{PreAF}}
%\newcommand{\oursauto}{\textsc{PreAF}$_\text{EST}$}

% \newcommand{\ours}{FPA}
% \newcommand{\oursauto}{FPA$_\text{Est}$}
% \newcommand{\estimator}{FPAEstimator}
% \newcommand{\ourslong}{\textbf{F}actual \textbf{P}recision in \textbf{A}tomic level}

\newcommand{\ourScore}{\textsc{FActScore}}
\newcommand{\ourScores}{\textsc{FActScore}s}

\newcommand{\subjectLM}{LM$_\textsc{subj}$}
\newcommand{\evalLM}{LM$_\textsc{eval}$}

\newcommand{\sLabel}{\texttt{Supported}}
\newcommand{\nsLabel}{\texttt{Not-supported}}
\newcommand{\irLabel}{\texttt{Irrelevant}}

\newcommand{\sLabelShort}{\texttt{S}}
\newcommand{\nsLabelShort}{\texttt{NS}}
\newcommand{\irLabelShort}{\texttt{IR}}

\newcommand{\rtg}{Retrieve$\rightarrow$LM}
\newcommand{\rtgShort}{Retrv$\rightarrow$LM}

% \newcommand{\Accuracy}{Accuracy$_\textsc{micro}$}
\newcommand{\Fone}{F1$_\textsc{micro}$}

\usepackage{adjustbox}
\newcommand{\marktext}[2]{\adjustbox{bgcolor=#1}{\strut #2}}
\newcommand{\myblue}[1]{\marktext{blue!30}{\texttt{#1}}}
\newcommand{\mypink}[1]{\marktext{pink!70}{\texttt{#1}}}
\newcommand{\mypurple}[1]{\marktext{purple!30}{\texttt{#1}}}

\newcommand{\myskip}[1]{}


%%%%%% results

\newcommand{\alwaysS}{ 30.8 & 37.1 & 45.0 }
\newcommand{\alwaysNS}{ 35.7 & 29.1 & 15.5 }
\newcommand{\alwaysRandom}{ 50.5 & 50.2 & 43.2 }

\newcommand{\noContextQA}{ 56.5 & 48.8 & 32.5 }
\newcommand{\noContextFV}{ 57.3 & 55.3 & 41.7 }
\newcommand{\selfcheckQA}{ 65.3 & 63.2 & - }
\newcommand{\selfcheckFV}{ 68.0 & 61.9 & - }

\newcommand{\retrievalQA}{ 64.3 & 58.2 & 47.3 }
\newcommand{\retrievalFV}{ 78.9 & 71.4 & 69.2 }
\newcommand{\npm}{ 70.6 & 66.4 & \textbf{69.5} }
\newcommand{\retrievalFVnpm}{ \textbf{80.5} & \textbf{74.5} & 68.5 }


\newcommand{\noContextFVseven}{  &  &  }
\newcommand{\retrievalFVseven}{  &  &  }
\newcommand{\retrievalFVsevennpm}{  &  &  }

\newcommand{\noContextFVsixtyfive}{ 41.6 & 46.4 & 51.4 }
\newcommand{\retrievalFVsixtyfive}{ 63.0 & 60.5 & 63.5 }
\newcommand{\retrievalFVsixtyfivenpm}{ 78.5 & 73.1 & \textbf{71.4} }

\newcommand{\noContextFVchatgpt}{ 51.9 & 49.1 & 53.3 }
\newcommand{\selfcheckchatgpt}{ 77.7 & 70.6 & - }
\newcommand{\retrievalFVchatgpt}{ \best{86.8} & \best{84.0} & \best{78.7} }
\newcommand{\retrievalFVchatgptnpm}{ \best{86.8} & 83.4 & 77.7 }

%%% sent-level

\newcommand{\noContextFVSent}{ 32.2 & 38.0 & 49.8 }
\newcommand{\retrievalFVSent}{ 53.5 & 46.6 & 56.6 }
\newcommand{\retrievalFVnpmSent}{ 66.8 & 62.0 & \underline{\textbf{68.9}} }

\newcommand{\noContextFVSentGenerated}{ 57.5 & 56.8 & 39.8 }
\newcommand{\retrievalFVSentGenerated}{ 71.8 & 67.0 & 63.9 }
\newcommand{\retrievalFVnpmSentGenerated}{ \textbf{75.0} & \textbf{70.2} & 66.3 }

\newcommand{\noContextFVSentOracle}{ 56.5 & 55.3 & 36.7 }
\newcommand{\retrievalFVSentOracle}{ 74.5 & 67.5 & 65.2 }
\newcommand{\retrievalFVnpmSentOracle}{ \underline{76.9} & \underline{71.7} & 67.5 }


\newcommand{\retrievalFVchatgptSent}{ 72.7 & 66.2 & 73.4 }
\newcommand{\retrievalFVchatgptnpmSent}{ 73.6 & 67.7 & 74.1 }

\newcommand{\retrievalFVchatgptSentGenerated}{ 81.4 & \best{80.3} & \best{76.6}  }
\newcommand{\retrievalFVchatgptnpmSentGenerated}{ \best{81.6} & 80.3 & 76.4 }

\newcommand{\retrievalFVchatgptSentOracle}{ \underline{84.6} & 81.8 & \underline{77.4} }
\newcommand{\retrievalFVchatgptnpmSentOracle}{ 84.4 & \underline{82.0} & \underline{77.4} }








==> Table/experment_instruct.tex <==



\begin{table*}[ht]
	\small
	\centering
	\begin{tabular}{p\textwidth}
		\toprule
            \rowcolor{tGold}{\fontfamily{ppl}\selectfont
            I want you to act as a \"fallacy finder\". You will be on the lookout for invalid arguments so you can call out any logical errors or inconsistencies that may be present in the \#Query\# and the \#Response\#. Your job is to provide evidence-based feedback and point out any fallacies, faulty reasoning, false assumptions, or incorrect conclusions which may be present in the \#Query\# and the \#Response\#. Begin your response with either FACTUAL or NON-FACTUAL, followed by your justification.} \\
       {\fontfamily{ppl}\selectfont \textbf{\#Query \#:} <Here is the query for the LLM >} \\
        {\fontfamily{ppl}\selectfont \textbf{\#Response \#:} <Here is the response from the LLM according to above query>} \\
            \bottomrule
	\end{tabular}
	\caption{Prompts for zero-shot evaluation. The role description is indicated by the \colorbox{tGold}{yellow} text.} 
        % \vspace{-0.2cm}
	\label{tab:prompt1}
\end{table*}



\begin{table*}[ht]
	\small
	\centering
	\begin{tabular}{p\textwidth}
		\toprule
            \rowcolor{tGold}{\fontfamily{ppl}\selectfont
            I want you to act as a \"fallacy finder\". You will be on the lookout for invalid arguments so you can call out any logical errors or inconsistencies that may be present in the \#Query\# and the \#Response\#. Your job is to provide evidence-based feedback and point out any fallacies, faulty reasoning, false assumptions, or incorrect conclusions which may be present in the \#Query\# and the \#Response\#. Begin your response with either FACTUAL or NON-FACTUAL, followed by your justification.} \\
            % \rowcolor{tPink}{\fontfamily{ppl}\selectfont You are trying to answer a question but there is a factual contradiction between the answer and the knowledge. You can fabricate some information that does not exist in the provided knowledge.} \\
            \specialrule{0em}{1pt}{1pt}
            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Query\#:} Which city is London twinned with?
            }\\ 
             \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Response\#:} London is twinned with *New York City*.
            }\\ 

            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Output\#:} FACTUAL.The response that London is twinned with New York City is correct. This is supported by the evidence that London is twinned with the administrative body of New York City. Therefore, there are no fallacies, faulty reasoning, or incorrect conclusions present in this query and response.
            }\\ 

            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Response\#:} London is twinned with *New York City*.
            }\\ 

             \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{} 
            }\\ 

             \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{ \#Query\#:} Which country has the highest total fertility rate in 1999?
            }\\ 

            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Response\#:} Zambia has the highest total fertility rate in 1999.
            }\\
            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Output\#:} The response that Zambia has the highest total fertility rate in 1999 is correct. According to the evidence provided, the total fertility rate for Zambia in 1999 was 6.116, which is the highest among all the countries listed. Therefore, there are no fallacies, faulty reasoning, or incorrect conclusions present in this query and response.
            }\\
            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{} 
            }\\
            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Query\#:}  What is the IETF language tag for the variety of English used in \"Land of the Lost\"?
            }\\
            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Response\#:} The IETF language tag for the variety of English used in \"Land of the Lost\" is *en-GB*.
            }\\
            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Output\#:} NON-FACTUAL.The response stating that the IETF language tag for the variety of English used in \"Land of the Lost\" is en-GB is incorrect. \"Land of the Lost\" uses the English language, which has a part called Australian English. The IETF language tag for Australian English is en-AU, not en-GB. Therefore, there is an incorrect conclusion in this query and response.
            }\\
            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{} 
            }\\
            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Query\#:} What is the IETF language tag for the part of English that Robert Young speaks, writes, or signs in?
            }\\
            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Response\#:} The IETF language tag for the part of English that Robert Young speaks, writes, or signs in is *en-GB*.
            }\\
            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Output\#:} NON-FACTUAL.The response stating that the IETF language tag for the part of English that Robert Young speaks, writes, or signs in is en-GB is incorrect. Robert Young speaks, writes, or signs in English, which has a part called Australian English. The IETF language tag for Australian English is en-AU, not en-GB. Therefore, there is an incorrect conclusion in this query and response.
            }\\

                  {\fontfamily{ppl}\selectfont 
                  \textbf{\# Query \#}: <Here is the query for the LLM>}\\
    {\fontfamily{ppl}\selectfont  \textbf{\# Response \#}: <Here is the response from the LLM according to above query>} \\
            \bottomrule
	\end{tabular}
	\caption{Prompts for few-shot evaluation.  Note that the demonstration only adopted in ICL(4-shot) setting. Large language models are known to be highly sensitive to prompts, especially in zero-shot and in-context learning settings. Therefore, we cannot guarantee that the prompts we used in the evaluation of FACTLLM are optimal. The role description is indicated by the \colorbox{tGold}{yellow} text, the evaluation demonstration is represented by the \colorbox{tGreen}{purple} text.} 
        % \vspace{-0.2cm}
	\label{tab:prompt2}
\end{table*}

==> Table/instruct1.tex <==
\begin{table*}[]
	\small
	\centering
	\begin{tabular}{p\textwidth}
		\toprule
            \rowcolor{tGold}{\fontfamily{ppl}\selectfont
           I want you to act as a question generator, your job is to generate questions with a *request* tone based on a given \#Response\#. Here are some examples:} \\
            % \rowcolor{tPink}{\fontfamily{ppl}\selectfont You are trying to answer a question but there is a factual contradiction between the answer and the knowledge. You can fabricate some information that does not exist in the provided knowledge.} \\
            \specialrule{0em}{1pt}{1pt}
            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Response\#:} Chris Terrio is an American.} \\
            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Query\#:} Please tell me which country Chris Terri is from?} \\
             \specialrule{0em}{1pt}{1pt}
                 \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Response\#:} The Renaissance was not a period in European history.} \\
            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Query\#:} Could you clarify whether the Renaissance was a period in European history?} \\
            \specialrule{0em}{1pt}{1pt}
            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Response\#:} Quantum computing is a type of computation that uses quantum mechanics to process information.} \\
            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Query\#:} Would you kindly explain what quantum computing is?} \\
            \specialrule{0em}{1pt}{1pt}
          \rowcolor{tBlue}{\fontfamily{ppl}\selectfont          You need to thoroughly study the above example to grasp the meaning of conventional Factuality. Please generate a complex and fluent query for the response without introducing any prior knowledge or the knowledge from the example. Make sure that the generated \#Query\# involve user instruction tone.  Follow the example format for output:} \\
          \\
             {\fontfamily{ppl}\selectfont \textbf{\#Response \#:} <Here is the claims with FACTUAL (SUPPORTS) or NON-FACTUAL (REFUTES) label from FEVER-like dataset and we need to leverage it for generating "\textsc{Query-Response}" contexts >} \\
            \bottomrule
	\end{tabular}
	\caption{Instruction for generating the ``\textsc{Query-Response}'' context based on FEVER-like dataset with the vanilla factuality pattern. The role description is indicated by the \colorbox{tGold}{yellow} text, the factuality demonstration is represented by the \colorbox{tGreen}{purple} text, while the factuality pattern is descripited by the  \colorbox{tBlue}{blue} text.} 
        % \vspace{-0.2cm}
	\label{tab:instruction11}
\end{table*}





\begin{table*}[t]
	\small
	\centering
	\begin{tabular}{p\textwidth}
		\toprule
            \rowcolor{tGold}{\fontfamily{ppl}\selectfont
            I want you to act as a complex and fluent question and answer data generator, where your task is to generate complex and fluent questions and answers that require multi-hop reasoning based entirely on the given knowledge. Here are some examples:} \\
            % \rowcolor{tPink}{\fontfamily{ppl}\selectfont You are trying to answer a question but there is a factual contradiction between the answer and the knowledge. You can fabricate some information that does not exist in the provided knowledge.} \\
            \specialrule{0em}{1pt}{1pt}
            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Knowledge\#:} ["Yao Ming", "spouse", "Ye Li"], ["Ye Li", "educated at", "Shanghai University of Sport"], ["Shanghai University of Sport", "establishment time", "November 1952"]} \\
            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Explanation\#:} To generate a question and answer, we need to perform multi-hop reasoning through the given knowledge. Here is the step-by-step reasoning: 
            
            1. Yao Ming's wife is named Ye Li.
            
            2. Ye Li was educated at Shanghai University of Sport.
            
            3. Shanghai University of Sport was established in November 1952.
            
            Based on the above reasoning chain, we can generate a complex question and answer with *3-hop* reasoning capabilities:} \\
             % \specialrule{0em}{1pt}{1pt}
            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Query\#:} Please tell me, when was the university that Yao Ming's wife graduated from established? } \\
            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Correct response\#:} Yao Ming's wife, Ye Li, graduated from Shanghai University of Sport, which was established in November 1952. } \\
            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Incorrect response\#:} Yao Ming's wife, Ye Li, graduated from Shanghai University of Sport, which was established in March 1954. } \\
            \specialrule{0em}{1pt}{1pt}
           \rowcolor{tGreen}{\fontfamily{ppl}\selectfont 
           <Demonstrations>} \\
            \specialrule{0em}{1pt}{1pt}
          \rowcolor{tBlue}{\fontfamily{ppl}\selectfont          You need to thoroughly study the above example to grasp the meaning of multi-hop reasoning, the core is step-by-step reasoning*. Please generate a complex and fluent query and response that requires multi-hop reasoning based entirely on the given knowledge below without introducing any prior knowledge or the knowledge from the example. Make sure that the generated \#Query\# involve multi-hop reasoning and include *all* the information from the \#Knowledge\#! Response include \#Correct response\# and \#Incorrect response\#. Make ensure that the \#Correct response\# can be *correctly* deduced from the \#Knowledge\# using multi-hop reasoning without relying on unknown or insufficient information. \#Incorrect response\# sounds plausible but is factually incorrect. *To produce \#Incorrect response\#, you should choose one or more of the following strategies: fabricate information to resolve factual contradictions, misunderstand the question context and intention, provide an answer that is either too general or too specific, or employ incorrect reasoning to arrive at a hallucinated answer not supported by the knowledge. Follow the example format for output:} \\
          \\
                  {\fontfamily{ppl}\selectfont \textbf{\#Knowledge \#:} <Here is the Knowledge we need to leverage for generating "\textsc{Query-Response}" contexts >} \\
            \bottomrule
	\end{tabular}
	\caption{Instruction for generating the ``\textsc{Query-Response}'' context based on KG with the multi-hop reasoning pattern. The role description is indicated by the \colorbox{tGold}{yellow} text, the factuality demonstration is represented by the \colorbox{tGreen}{purple} text, while the factuality pattern is descripited by the  \colorbox{tBlue}{blue} text.} 
        % \vspace{-0.2cm}
	\label{tab:instruction12}
\end{table*}



\begin{table*}[t]
	\small
	\centering
	\begin{tabular}{p\textwidth}
		\toprule
            \rowcolor{tGold}{\fontfamily{ppl}\selectfont
            I want you to act as a complex and fluent question and answer data generator, where your task is to generate a complex and fluent question and answer that require quantitative comparison, relying solely on the provided knowledge. Here are some examples:} \\
            % \rowcolor{tPink}{\fontfamily{ppl}\selectfont You are trying to answer a question but there is a factual contradiction between the answer and the knowledge. You can fabricate some information that does not exist in the provided knowledge.} \\
            \specialrule{0em}{1pt}{1pt}
            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Knowledge\#:} ["Chris Paul", "instance of", "human"], ["Chris Paul", "height", "183 centimetre"], ["Franklin Delano Roosevelt", "instance of", "human"], ["Franklin Delano Roosevelt", "height", "189 centimetre"]} \\
             % \specialrule{0em}{1pt}{1pt}
            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Query\#:} Could you kindly tell me who is taller, Chris Paul or Franklin Delano Roosevelt, both of whom are human?} \\
            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Correct response\#:} Franklin Delano Roosevelt is taller than Chris Paul. Roosevelt's height is 189 centimeters while Chris Paul's height is 183 centimeters. } \\
            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Incorrect response\#:} Chris Paul is taller than Franklin Delano Roosevelt. Chris Paul's height is 183 centimeters while Roosevelt's height is 189 centimeters.} \\
            \specialrule{0em}{1pt}{1pt}
           \rowcolor{tGreen}{\fontfamily{ppl}\selectfont 
           <Demonstrations>} \\
            \specialrule{0em}{1pt}{1pt}
          \rowcolor{tBlue}{\fontfamily{ppl}\selectfont       You need to thoroughly study the above example to grasp the meaning of quantitative comparison. Please generate a complex and fluent query and response that requires quantitative comparison based entirely on the given knowledge below without introducing any prior knowledge or the triplets from the example. Make sure that the generated \#Query\# involve quantitative comparison and include all the information from the \#Knowledge\#! Answers include \#Correct response\# and \#Incorrect response\#. Make ensure that the \#Correct response\# can be *correctly* deduced from the \#Knowledge\# using quantitative comparison without relying on unknown or insufficient information. \#Incorrect response\# sounds plausible but is factually incorrect. To produce \#Incorrect response\#, you should choose one or more of the following strategies: fabricate information to resolve factual contradictions, misunderstand the question context and intention, provide an answer that is either too general or too specific, or employ incorrect reasoning to arrive at a hallucinated answer not supported by the knowledge. Follow the example format for output:} \\
          \\
                  {\fontfamily{ppl}\selectfont \textbf{\#Knowledge \#:} <Here is the Knowledge we need to leverage for generating "\textsc{Query-Response}" contexts >} \\
            \bottomrule
	\end{tabular}
	\caption{Instruction for generating the ``\textsc{Query-Response}'' context based on KG with the comparing fact. The role description is indicated by the \colorbox{tGold}{yellow} text, the factuality demonstration is represented by the \colorbox{tGreen}{purple} text, while the factuality pattern is descripited by the  \colorbox{tBlue}{blue} text.} 
        % \vspace{-0.2cm}
	\label{tab:instruction13}
\end{table*}



\begin{table*}[t]
	\small
	\centering
	\begin{tabular}{p\textwidth}
		\toprule
            \rowcolor{tGold}{\fontfamily{ppl}\selectfont
            I want you to act as a complex and fluent question and answer data generator, where your task is to generate a complex and fluent question and answer that require set operation, relying solely on the provided knowledge. Here are some examples:} \\
            % \rowcolor{tPink}{\fontfamily{ppl}\selectfont You are trying to answer a question but there is a factual contradiction between the answer and the knowledge. You can fabricate some information that does not exist in the provided knowledge.} \\
            \specialrule{0em}{1pt}{1pt}
            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Knowledge\#:} ["Mission: Impossible II", "producer", "Tom Cruise"], ["Mission: Impossible II", "original language of film or TV show", "English"], ["Mission: Impossible II", "composer", "Hans Zimmer"], ["The Last Samurai", "producer", "Tom Cruise"], ["The Last Samurai", "original language of film or TV show", "English"], ["The Last Samurai", "composer", "Hans Zimmer"]} \\
             % \specialrule{0em}{1pt}{1pt}
            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Query\#:}Could you provide the names of films produced by Tom Cruise, composed by Hans Zimmer, and with English as the original language of the film or TV show?} \\
            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Correct response\#:} The films that meet the given criteria are "Mission: Impossible II" and "The Last Samurai." } \\
            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Incorrect response\#:} The films that meet the given criteria are "Top Gun" and "Jerry Maguire."} \\
            \specialrule{0em}{1pt}{1pt}
           \rowcolor{tGreen}{\fontfamily{ppl}\selectfont 
           <Demonstrations>} \\
            \specialrule{0em}{1pt}{1pt}
          \rowcolor{tBlue}{\fontfamily{ppl}\selectfont       You need to thoroughly study the above example to grasp the meaning of set operation. Please generate a complex and fluent query and response that requires set operation based entirely on the given knowledge below without introducing any prior knowledge or the triplets from the example. Make sure that the generated \#Query\# involve set operation and include all the information from the \#Knowledge\#! Answers include \#Correct response\# and \#Incorrect response\#. Make ensure that the \#Correct response\# can be *correctly* deduced from the \#Knowledge\# using set operation without relying on unknown or insufficient information. \#Incorrect response\# sounds plausible but is factually incorrect. To produce \#Incorrect response\#, you should choose one or more of the following strategies: fabricate information to resolve factual contradictions, misunderstand the question context and intention, provide an answer that is either too general or too specific, or employ incorrect reasoning to arrive at a hallucinated answer not supported by the knowledge. Follow the example format for output:} \\
          \\
                  {\fontfamily{ppl}\selectfont \textbf{\#Knowledge \#:} <Here is the Knowledge we need to leverage for generating "\textsc{Query-Response}" contexts >} \\
            \bottomrule
	\end{tabular}
	\caption{Instruction for generating the ``\textsc{Query-Response}'' context based on KG with the set operation. The role description is indicated by the \colorbox{tGold}{yellow} text, the factuality demonstration is represented by the \colorbox{tGreen}{purple} text, while the factuality pattern is descripited by the  \colorbox{tBlue}{blue} text.} 
        % \vspace{-0.2cm}
	\label{tab:instruction14}
\end{table*}



==> Table/instruct2.tex <==
\begin{table*}[ht]

 \centering
 \tiny
 \scalebox{0.85}{
	\begin{tabular}{p\textwidth}
		\toprule
            \rowcolor{tGold}{\fontfamily{ppl}\selectfont
            
            I want you to act as a data generator for a fallacy-finding task. You will be on the lookout for invalid arguments so you can call out any logical errors or inconsistencies that may be present in \#Question\# and \#Answer\#. I'll tell you the right label: FACTUAL or NON-FACTUAL. Your job is to provide rational evidence-based feedback and point out any fallacies, faulty reasoning, false assumptions, or incorrect conclusions that may be present in the \#Question\# and \#Answer\#. Here are some examples:} \\
            % \rowcolor{tPink}{\fontfamily{ppl}\selectfont You are trying to answer a question but there is a factual contradiction between the answer and the knowledge. You can fabricate some information that does not exist in the provided knowledge.} \\
      
            \specialrule{0em}{1pt}{1pt}
           \rowcolor{tGreen}{\fontfamily{ppl}\selectfont  \textbf{\#Golden Label\#:} \colorbox{tPurple}{NON-FACTUAL}} \\
            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Query\#:} How many children did the leader of the country, where the distributor of "The Killer Inside Me" operates, have?} \\
            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Response\#:} The head of government of the United States of America, John F. Kennedy, had 2 children. } \\
            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Evidence\#:}  ["The Killer Inside Me", "distributor", "Warner Bros."], ["Warner Bros.", "owner of", "Warner Bros. Animation"], ["Warner Bros. Animation", "country", "United States of America"], ["United States of America", "head of government", "John F. Kennedy"], ["John F. Kennedy", "number of children", "4"]} \\
            \rowcolor{tGreen}{\fontfamily{ppl}\selectfont \textbf{\#Output\#:} NON-FACTUAL.
            The answer stating that the head of government of the United States of America, John F. Kennedy, had 2 children is incorrect. "The Killer Inside Me" is distributed by Warner Bros., which is the owner of Warner Bros. Animation. Warner Bros. Animation is located in the United States of America, where the head of government was John F. Kennedy. However, John F. Kennedy had 4 children, not 2. Therefore, there is an incorrect conclusion in this query and response.} \\     
    \specialrule{0em}{1pt}{1pt}
    \rowcolor{tGreen}{\fontfamily{ppl}\selectfont 
           <Demonstrations>} \\ 
            
            \specialrule{0em}{1pt}{1pt}
            {\fontfamily{ppl}\selectfont \textbf{\#Golden Lable\#:} <Here is the right label for the factuality of the following sample >} 
            {\fontfamily{ppl}\selectfont \textbf{\#Query\#:} <Here is the query for the LLM> } 
            {\fontfamily{ppl}\selectfont \textbf{\#Response\#:} <Here is the response from the LLM according to the above query>} 
             {\fontfamily{ppl}\selectfont \textbf{\#Evidence\#:} <Here is the evidence with fact to judge the factuality of above context>} \\
            {\fontfamily{ppl}\selectfont \textbf{\#Output\#:}} \\
            \bottomrule
	\end{tabular}}
 	\caption{Instruction to generate evidence-based chains of facts for the ``\textsc{Query-Response}'' contexts. The role description is indicated by the \colorbox{tGold}{yellow} text, while the factuality demonstration is represented by the \colorbox{tGreen}{purple} text.} 
        % \vspace{-0.2cm}
	\label{tab:instruction2}
\end{table*}

